Generative Modelling with Tensor Train approximations of Hamilton--Jacobi--Bellman equations

Sampling from probability densities is a common challenge in fields such as Uncertainty Quantification (UQ) and Generative Modelling (GM). In GM in particular, the use of reverse-time diffusion processes depending on the log-densities of Ornstein-Uhlenbeck forward processes are a popular sampling tool. In Berner et al. [2022] the authors point out that these log-densities can be obtained by solution of a \textit{Hamilton-Jacobi-Bellman} (HJB) equation known from stochastic optimal control. While this HJB equation is usually treated with indirect methods such as policy iteration and unsupervised training of black-box architectures like Neural Networks, we propose instead to solve the HJB equation by direct time integration, using compressed polynomials represented in the Tensor Train (TT) format for spatial discretization. Crucially, this method is sample-free, agnostic to normalization constants and can avoid the curse of dimensionality due to the TT compression. We provide a complete derivation of the HJB equation's action on Tensor Train polynomials and demonstrate the performance of the proposed time-step-, rank- and degree-adaptive integration method on a nonlinear sampling task in 20 dimensions.

==> 02_Methodology.tex <==
\section{Time stepping solution of HJB \& Dynamical Low Rank approximation}

\subsection{Solving HJB}
\begin{itemize}
    \item HJB formalism
    \item Problem of explicit solvers
    \item implicit formalism and fitting formulation and algorithm
\end{itemize}









==> 03_theory.tex <==
\section{Theoretical results}


\begin{itemize}
    \item Gradient accuracy in the fitting through connection of the optimal control problem with the value function and associated gradient 
    \item Accuracy of the value function fit
    \item Distance in distribution of our learned solution to the posterior, error on control of $V_t$ implies what?
    \item Get an error result for the resulting distribution in spirit of the Jakiw Paper. 
    % \includegraphics[width = 0.8\linewidth]{images/screenshot_jakiw.png}
    \item influcence in the errror progation of the time reverse SDE maybe in the spirit of Jentzen Paper
    % \begin{center}
    % \includegraphics[width = 0.8\linewidth]{images/screenschot_jentzen.png}
    % \end{center}
    The Jentzen seems directly be applicable to the time reverse SDE setup
    \item Instead consider the case of ODEs and apply perturbation of ODEs to describe distribution
    \begin{itemize}
        \item Different start values of distribution ($x(T)$ and Gaussian)
        \item Effect of perturbed $\tilde{V}_t\approx V_t$ within the ODE propagation and effect of resulting distribution
        \item time discretization of the ODE
    \end{itemize}

   

\end{itemize}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
